Spectral Element Simulation of Liquid Metal Magnetohydrodynamics

A spectral-element-based formulation of incompressible MHD is presented in the context of the open-source fluid-thermal code, Nek5000/RS. The formulation supports magnetic fields in a solid domain that surrounds the fluid domain. Several steady-state and time-transient model problems are presented as part of the code verification process. Nek5000/RS is designed for large-scale turbulence simulations, which will be the next step with this new MHD capability.

==> tex/paul_figs.tex <==


% \begin{figure}    
% \centering
%     \includegraphics[width=0.95\textwidth]{./figs/p_vc1.png}
%     \\                                   
%     (a) $\sigma_w= 10^5$, $B_0=$ 10, 50, 100. 
%     \vspace{1.em}
%     \\                                   
%     \includegraphics[width=0.95\textwidth]{./figs/p_vc2.png}
%     \\                                   
%     (b) $\sigma_w= 1$, $B_0=$ 10, 50, 100. 
%     \vspace{1.em}
%     \\                                   
%     \includegraphics[width=0.95\textwidth]{./figs/p_vc3.png}
%     \\
%     (c)  $\sigma_w= 10^{-5}$, $B_0=$ 10, 50, 100. 
%     \vspace{1.em}
%     \caption{Velocity distribution contour for 
%              (a) $\sigma_w= 10^5$, (b) $\sigma_w= 1$, and (c) $\sigma_w= 10^{-5}$ (bottom). 
%              $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.} 
% \label{vcontour}
% \end{figure}


% \begin{figure}
% \centering
%     \includegraphics[width=1.\textwidth]{./figs/p_v1.png}
%     \\
%     (a) $\sigma_w= 10^5$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=1.\textwidth]{./figs/p_v2.png}
%     \\
%     (b) $\sigma_w= 1$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=1.\textwidth]{./figs/p_v3.png}
%     \\
%     (c) $\sigma_w= 10^{-5}$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \caption{Velocity distribution profile for
%             (a) $\sigma_w= 10^5$, (b) $\sigma_w= 1$, and (c) $\sigma_w= 10^{-5}$ (bottom).
%              $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
% \label{vmesh}
% \end{figure}


% \begin{figure}
% \centering
%     \includegraphics[width=0.95\textwidth]{./figs/p_mc1.png}
%     \\
%     (a) $\sigma_w= 10^5$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=0.95\textwidth]{./figs/p_mc2.png}
%     \\
%     (b) $\sigma_w= 1$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=0.95\textwidth]{./figs/p_mc3.png}
%     \\
%     (c) $\sigma_w= 10^{-5}$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \caption{Magnetic distribution contour for
%              (a) $\sigma_w= 10^5$, (b) $\sigma_w= 1$, and (c) $\sigma_w= 10^{-5}$ (bottom).
%              $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
% \label{bcontour}
% \end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[t]{0.3\textwidth} % Width specification added
        \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
        $\begin{matrix}
            \sigma_w \\ 10^{2}
        \end{matrix}$
        }}}%
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha010vel.png}\\[5pt]
        \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
        $\begin{matrix}
            \sigma_w \\ 1
        \end{matrix}$
        }}}%
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha010vel.png}\\[5pt]
        \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
        $\begin{matrix}
            \sigma_w \\ 10^{-5}
        \end{matrix}$
        }}}%
        \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha010vel.png}
        \caption{$\ha = 10$} % Added caption
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth} % Width specification added
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha050vel.png}\\[5pt]
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha050vel.png}\\[5pt]
        \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha050vel.png}
        \caption{$\ha = 50$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth} % Width specification added
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha100vel.png}\\[5pt]
        \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha100vel.png}\\[5pt]
        \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha100vel.png}
        \caption{$\ha = 100$} % Added caption
    \end{subfigure}
    \caption{Velocity distribution profile for
             $\sigma_w= 10^5$,  $\sigma_w= 1$, and  $\sigma_w= 10^{-5}$ (bottom).
             $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
    \label{vmesh}
\end{figure}


\begin{figure}
  \centering
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 10^{2}
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha010velcont.png}\\[5pt]
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 1
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha010velcont.png}\\[5pt]
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 10^{-5}
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha010velcont.png}
      \caption{$\ha = 10$} % Added caption
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha050velcont.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha050velcont.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha050velcont.png}
      \caption{$\ha = 50$}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha100velcont.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha100velcont.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha100velcont.png}
      \caption{$\ha = 100$} % Added caption
  \end{subfigure}
  \caption{Velocity distribution contour for 
   $\sigma_w= 10^5$,  $\sigma_w= 1$, and $\sigma_w= 10^{-5}$ (bottom). 
  $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.} 
  \label{vcontour}
\end{figure}


\begin{figure}
  \centering
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 10^{2}
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha010mgn.png}\\[5pt]
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 1
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha010mgn.png}\\[5pt]
      \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
      $\begin{matrix}
          \sigma_w \\ 10^{-5}
      \end{matrix}$
      }}}%
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha010mgn.png}
      \caption{$\ha = 10$} % Added caption
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha050mgn.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha050mgn.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha050mgn.png}
      \caption{$\ha = 50$}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth} % Width specification added
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha100mgn.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha100mgn.png}\\[5pt]
      \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha100mgn.png}
      \caption{$\ha = 100$} % Added caption
  \end{subfigure}
  \caption{Magnetic distribution profile for
  $\sigma_w= 10^5$,  $\sigma_w= 1$, and  $\sigma_w= 10^{-5}$ (bottom).
  $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
  \label{bmesh}
\end{figure}


\begin{figure}
\centering
\begin{subfigure}[t]{0.3\textwidth} % Width specification added
    \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
    $\begin{matrix}
        \sigma_w \\ 10^{2}
    \end{matrix}$
    }}}%
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha010mgncont.png}\\[5pt]
    \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
    $\begin{matrix}
        \sigma_w \\ 1
    \end{matrix}$
    }}}%
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha010mgncont.png}\\[5pt]
    \makebox[20pt]{\raisebox{40pt}{\rotatebox[origin=c]{0}{
    $\begin{matrix}
        \sigma_w \\ 10^{-5}
    \end{matrix}$
    }}}%
    \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha010mgncont.png}
    \caption{$\ha = 10$} % Added caption
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\textwidth} % Width specification added
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha050mgncont.png}\\[5pt]
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha050mgncont.png}\\[5pt]
    \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha050mgncont.png}
    \caption{$\ha = 50$}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.3\textwidth} % Width specification added
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp5ha100mgncont.png}\\[5pt]
    \includegraphics[width=\textwidth]{figs/nekrs_result/sp0ha100mgncont.png}\\[5pt]
    \includegraphics[width=\textwidth]{figs/nekrs_result/sm5ha100mgncont.png}
    \caption{$\ha = 100$} % Added caption
\end{subfigure}
\caption{Magnetic distribution contour for
$\sigma_w= 10^5$, $\sigma_w= 1$, and $\sigma_w= 10^{-5}$ (bottom).
$B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
\label{bcontour}
\end{figure}

% \begin{figure}
% \centering
%     \includegraphics[width=1.\textwidth]{./figs/p_m1.png}
%     \\
%     (a) $\sigma_w= 10^5$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=1.\textwidth]{./figs/p_m2.png}
%     \\
%     (b) $\sigma_w= 1$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \\
%     \includegraphics[width=1.\textwidth]{./figs/p_m3.png}
%     \\
%     (c) $\sigma_w= 10^{-5}$, $B_0=$ 10, 50, 100.
%     \vspace{1.em}
%     \caption{Magnetic distribution profile for
%              (a) $\sigma_w= 10^5$, (b) $\sigma_w= 1$, and (c) $\sigma_w= 10^{-5}$ (bottom).
%              $B_0=\ha/\sqrt{Re * Rm}$= 10, 50, and 100 are used from left to right.}
% \label{bmesh}
% \end{figure}

%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.7\textwidth]{./figs/centerptvalue.eps}
%\caption{Time history of center-point velocity for $Ha=50, Re=1, Rm=1$. }
%\label{rerm1}
%\end{figure}
 
% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re05Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=0.5, Rm=1$. }
% \label{re05rm1}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re2Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=2, Rm=1$. }
% \label{re2rm1}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re10Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=10, Rm=1$. }
% \label{re10rm1}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re100Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=100, Rm=1$. }
% \label{re100rm1}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re10000Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=10000, Rm=1$. }
% \label{re10000rm1}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.7\textwidth]{./figs/Re100000Rm1.eps}
% \caption{Time history of center-point velocity for $Ha=50, Re=100000, Rm=1$. }
% \label{re100000rm1}
% \end{figure}








==> tex/preambl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geometry 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{geometry}
%\geometry{left   = 1.0in,
%          right  = 1.0in,
%          top    = 1.0in,
%          bottom = 1.0in}

\usepackage{moreverb,url}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{graphicx}
\usepackage{rotating}

\usepackage{setspace}
\usepackage{lipsum}
%\newcommand{\verbatimfont}[1]{\renewcommand{\verbatim@font}{\ttfamily#1}}
\usepackage{epstopdf}
\usepackage{alltt}
\usepackage{color}
\usepackage{multirow}
\usepackage{listings}

\usepackage{fancyvrb}
\fvset{fontsize=\scriptsize}
%\fvset{fontsize=\footnotesize}
\RecustomVerbatimEnvironment{verbatim}{Verbatim}{}

\usepackage{floatrow}
\floatsetup[table]{capposition=top}
\usepackage{algpseudocode,algorithm,algorithmicx}
%\usepackage{algcompatible}
\usepackage{todonotes}

\usepackage[per-mode=symbol]{siunitx}
\usepackage{pgfplots}
%\pgfplotsset{compat=1.17}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formats
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{pgfplots,epsf,graphicx,color}
\usepackage{amsmath,amsfonts,amsthm,multirow}

\usepackage{comment}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage{float}

\usepackage{pdfpages}
\usepackage{afterpage}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{fullpage}
\usepackage{bm} 
\usepackage{caption} 
\usepackage{etoolbox}
\usepackage{pgfplots}
\usepackage{subcaption}
\pgfplotsset{compat=newest}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[colorlinks=true]{hyperref}
\hypersetup{
  colorlinks  = true, %Colours links instead of ugly boxes
  urlcolor    = blue, %Colour for external hyperlinks
  linkcolor   = blue, %Colour of internal links
  citecolor   = blue, %Colour of citations
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epstopdf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newif\ifpdf
%\ifx\pdfoutput\undefined
%   \pdffalse
%\else
%   \pdfoutput=1
%   \pdftrue
%\fi
%\ifpdf
%   \usepackage[update,prepend]{epstopdf}
%   \DeclareGraphicsRule{.eps}{pdf}{.pdf}{`epstopdf #1}
%   \pdfcompresslevel=9
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{authblk}
\usepackage{chngcntr}
\usepackage{./sty/mcs_pack}

\DeclareGraphicsExtensions{.gif,.png,.jpg,.pdf,.tiff,.eps}	

\def\baselinestretch{1.0}
\textwidth 6.5in
\textheight 8.50in
\topmargin -0.15in
\parskip   0.05in
\oddsidemargin 0.0in
\parindent 5ex
\renewcommand{\topfraction}{.95}
\renewcommand{\bottomfraction}{.95}
\renewcommand{\textfraction}{.05}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\VI{\bold{v}}
%\newcommand{\projectname}{SHARP Thermal-Hydraulics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




